Making Neural Networks More Suitable for Approximate Clifford+T Circuit Synthesis

Machine Learning with deep neural networks has transformed computational approaches to scientific and engineering problems. Central to many of these advancements are precisely tuned neural architectures that are tailored to the domains in which they are used. In this work, we develop deep learning techniques and architectural modifications that improve performance on reinforcement learning guided quantum circuit synthesis-the task of constructing a circuit that implements a given unitary matrix. First, we propose a global phase invariance operation which makes our architecture resilient to complex global phase shifts. Second, we demonstrate how augmenting data with small random unitary perturbations during training enables more robust learning. Finally, we show how encoding numerical data with techniques from image processing allow networks to better detect small but significant changes in data. Our work enables deep learning approaches to better synthesize quantum circuits that implement unitary matrices.

==> sections/acknowledgements.tex <==
The authors thank Sammuel Pfrommer for useful discussion about NeRF encodings.
This work was supported by the DOE under contract DE-5AC02-05CH11231 through the Office of Advanced Scientific Computing Research (ASCR) Quantum Algorithms Team and Accelerated Research in Quantum Computing programs.
This work was also supported by the NSF Challenge Institute for Quantum Computation (CIQC) program under award OMA-2016245 and through a CIQC seed funding award.

==> sections/diagonalization.tex <==
\label{sec:diagonalization}
Directly synthesizing a unitary by finding a sequence of gates which inverts it is intractable when high-precision is needed.
This is because a large number of discrete gates are required to implement any single continuous rotation.
To address this we shift the problem scope from inversion to diagonalization.
This approach assumes there are continuous degrees of freedom in unitaries which cannot be handled by a search-based synthesis process.
% Instead of synthesizing unitaries directly by matrix inversion we take the approach of diagonalization.
To fit the paradigm of search-based synthesis as described in Section~\ref{sec:synthesis}, we first define the problem of diagonalization as an MDP.
At time $t \in \{0, 1,\dots, T\}$ in the synthesis process, the state $\mdpstate{t} \in \statespace$ is defined by 
\begin{equation}
    \label{eqn:state}
    \mdpstate{t} = L_t \target^\dagger R_t
\end{equation}
where $L_t, R_t$ are each sequences of discrete operations (as in Equation~\ref{eqn:circuitunitary}).
The set of initial states contains the adjoint of target unitaries $S_I = \{ \target^\dagger \}$, meaning $R_0 = L_0 = I_{2^n}$.
The set of terminal states is the set of all states which can be approximately inverted by a diagonal unitary matrix.
This corresponds to the set of states satisfying
\begin{equation}
    \label{eqn:diagdistance}
    d_{D}(s_t) = \min_{\theta \in \realnum^{2^n}} d_{HS}\big(\mdpstate{t}, \exp(-i \theta \cdot \hat\sigma)\big) \leq \epsilon
\end{equation}
where $\hat\sigma$ is the vector of all $n$-fold tensor products of the Pauli $\sigma_I$ and $\sigma_Z$ matrices. For brevity's sake, we denote the diagonal operator resulting from the matrix exponential as $D_\theta$.
The reward function is an indicator function defined as
\begin{equation}
    \label{eqn:reward}
    r(\mdpstate{t}) = \begin{cases} 
      +1 & \text{if } \mdpstate{t} \in \terminalstates \\
      -1 & \text{else}
   \end{cases}
\end{equation}
Given a terminal state $s_T$, the corresponding circuit is
\begin{equation}
    R_T s_T^\dagger L_T = R_T D_\theta^{-1} L_T.
\end{equation}
Figure~\ref{fig:toffoli} illustrates the general form of three-qubit circuits which satisfy this structure. As an example, the Toffoli gate can be diagonalized by just two Hadamard gates.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/toffoli.pdf}
    \caption{
        Diagonalization ansatz for three-qubit unitaries.
        The diagonal matrix corresponds to $2^n$-$1$ continuous degrees of freedom which can be efficiently implemented with $R_Z(\theta)$ and CNOT gates.
        The $L$ and $R$ subcircuits are made of discrete Clifford+T operations.
        A Toffoli only requires two H gates to be diagonalized and its diagonalization can be implemented with only CNOT and $R_Z(\pm\frac{\pi}{4})$ ($T$ or $T^\dagger$ gates).
    }
    \label{fig:toffoli}
\end{figure}

This process can be be thought of as a Singular Value Decomposition where the left and right singular vector matrices are restricted to unitaries which can be efficiently implemented by searching through gate sequences from a discrete gate set (i.e. Clifford+T).
Although our implementation of synthesis by diagonalization uses RL, other search-based synthesis methods are equally valid.
A tool such as Synthetiq can be retrofitted to leverage diagonalization.

\subsection{Handling Diagonal Unitaries and Rotation Gates}
The diagonal operator $D_\theta$ captures continuous degrees of freedom that cannot be efficiently handled by the $L_t$ and $R_t$ unitaries.
An ansatz implementing $D_\theta$ can be prepared using specialized algorithms for synthesizing diagonal unitaries \cite{bullock_2004_diagonal, li_2022_paulihedral, welch_efficient_2014}.
These diagonal unitaries require only $CNOT$ and $R_Z$ gates.
In this paper, $R_Z$ rotations are implemented without ancilla in the Clifford+T gate set using \gridsynth{} \cite{ross_2016_gridsynth}, but alternative techniques can also be used.


==> sections/name.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c||c|}
    \hline
    \multirow{13}{*}{\rotatebox{90}{2 Qubits}} & & Heisenberg & HHL & Hubbard & QAOA & QPE & Shor & TFIM & VQE & Mean \\
    \hline
    & Success Rate & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\
    & & 93.7\% & 37.4\% & 42.8\% & 27.1\% & 29.1\% & 41.7\%  & 51.0\% & 20.0\% & 42.9\% \\
    \cline{2-11}
    & T Count  & 495.18 & 530.89 & 443.84 & 579.32 & 551.82 & 511.85 & 430.50 & 341.62 & 485.98\\
    &  & 70.03 & 115.16 & 59.50 & 74.20 & 64.85 & 109.30 & 70.00 & 65.96 & 78.63\\
    \cline{2-11}
    & Clifford Count & 711.66 & 762.20 & 638.63 & 832.15 & 792.35 & 736.77 & 617.06 & 491.33 & 698.27\\
    & & 104.39 & 168.01 & 88.16 & 108.10 & 94.50 & 160.07 & 105.47 & 102.31 & 116.38\\
    \cline{2-11}
    & T Reduction & \bf{85.9\%} & \bf{78.4\%} & \bf{86.6\%} & \bf{87.2\%} & \bf{88.5\%} & \bf{78.7\%} & \bf{83.7\%} & \bf{80.7\%} & \bf{83.5\%} \\
    \cline{2-11}
    \hline
    \hline
    \cline{2-11}
    \multirow{12}{*}{\rotatebox{90}{3 Qubits}} 
    & Success Rate & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\
    & & 27.4\% & 9.6\% & 55.6\% & 11.2\% & 78.5\% & 18.0\% & 9.4\% & 13.3\% & 27.9\% \\
    \cline{2-11}
    & T Count  & 3123.46 & 2130.08 & 2572.95 & 2168.42 & 3283.56 & 3058.70 & 2425.20 & 3051.74 & 2726.50\\
    &  & 131.70 & 146.35 & 61.37 & 158.90 & 107.14 & 294.98 & 133.17 & 50.83 & 135.29\\
    \cline{2-11}
    & Clifford Count  & 3601.85 & 2462.84 & 2972.88 & 2506.86 & 3786.61 & 3531.55 & 2800.35 & 3520.56 & 3147.64\\
    &  & 163.46 & 180.74 & 84.45 & 191.82 & 132.40 & 348.72 & 168.76 & 74.29 & 167.78\\
    \cline{2-11}
    & T Reduction & \bf{95.8\%} & \bf{93.2\%} & \bf{97.6\%} & \bf{92.7\%} & \bf{96.8\%} & \bf{90.4\%} & \bf{94.5\%} & \bf{98.3\%} & \bf{95.1\%} \\
    \cline{2-11}
    \hline
    \end{tabular}
    \caption{
        Synthesis of 2- and 3-qubit unitaries taken from partitioned circuits (see Figure~\ref{fig:transpilation} for an illustration).
        In both cases, each unitary is synthesized in approximately 1 second.
        When $R_Z$ gates appear due to the diagonalization process, they are synthesized using \emph{gridsynth}~\cite{ross_2016_gridsynth}. Each $R_Z$ gate is synthesized to a precision of $\epsilon=10^{-7}$ which results in approximately 70 T gates and 110 Clifford gates per $R_Z$.
        Numbers indicate average time, success rate, Clifford, and non-Clifford gate counts for unitaries taken from a variety of benchmarks.
        Compared to the QSD (top rows), the diagonalizing agent (bottom rows) on average reduces the number of $R_Z$ gates by 83.5\% and 95.1\% for 2- and 3-qubit unitaries respectively. 
        Comparisons are made to the QSD because other synthesis tools fail to find solutions given $\epsilon \leq 10^{-4}$.
    }
    \label{tab:qsd_comparison}
\end{table*}
